Descartes: Generating Short Descriptions of Wikipedia Articles

Wikipedia is one of the richest knowledge sources on the Web today. In order to facilitate navigating, searching, and maintaining its content, Wikipedia's guidelines state that all articles should be annotated with a so-called short description indicating the article's topic (e.g., the short description of beer is "Alcoholic drink made from fermented cereal grains"). Nonetheless, a large fraction of articles (ranging from 10.2% in Dutch to 99.7% in Kazakh) have no short description yet, with detrimental effects for millions of Wikipedia users. Motivated by this problem, we introduce the novel task of automatically generating short descriptions for Wikipedia articles and propose Descartes, a multilingual model for tackling it. Descartes integrates three sources of information to generate an article description in a target language: the text of the article in all its language versions, the already-existing descriptions (if any) of the article in other languages, and semantic type information obtained from a knowledge graph. We evaluate a Descartes model trained for handling 25 languages simultaneously, showing that it beats baselines (including a strong translation-based baseline) and performs on par with monolingual models tailored for specific languages. A human evaluation on three languages further shows that the quality of Descartes's descriptions is largely indistinguishable from that of human-written descriptions; e.g., 91.3% of our English descriptions (vs. 92.1% of human-written descriptions) pass the bar for inclusion in Wikipedia, suggesting that Descartes is ready for production, with the potential to support human editors in filling a major gap in today's Wikipedia across languages.

==> _UNUSED_03_wikidata.tex <==
Wikipedia short descriptions\footnote{\url{https://en.wikipedia.org/wiki/Wikipedia:Short_description}} provide a concise indication of the field covered by the article. Every article should eventually have one. By briefly summarizing the topic of the article, they act as short annotations and help disambiguate search results. Currently, short descriptions appear in Wikipedia mobile and some desktop searches, as well as under the page title in the mobile application. They do not appear in the desktop version of the page by default, but logged-in users can enable it. Short descriptions are bound to be more widely used within Wikipedia when the proportion of articles missing it drops.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\columnwidth]{images/wikidata_wikipedia.pdf}
    \caption{\textmd{\textbf{Statistics of short descriptions in Wikidata and Wikipedia.} For each language, the height of the bar represents the percentage of articles which have a Wikidata description but not a Wikipedia description. The number on top reports the percentage of articles for which the Wikipedia description and the Wikidata description are exact copies, when both are available. Languages are sorted in the same order as \Figref{fig:figure_1}.  }  %\maxime{Need Appref} %\maxime{TODO}.
    %(with $K$ standing for $10e3$). 
    }
    \label{fig:wikidata_stats}
\end{figure}


There exists a similar concept in Wikidata called \emph{Wikidata descriptions}\footnote{\url{https://www.wikidata.org/wiki/Help:Description}}. 
The purpose is to disambiguate Wikidata items with similar labels. One might be tempted to use Wikidata descriptions as Wikipedia ones and conversely which is often what editors have been doing in practice.
As shown by~\Figref{fig:wikidata_stats}, articles without short descriptions in Wikipedia, also don't have Wikidata descriptions; the best complementarity is for English where 4.2\% of articles that miss a Wikipedia description have one in Wikidata. Additionally, when both Wikipedia and Wikidata descriptions exist, they are generally the same, as shown by \Figref{fig:wikidata_stats}. Overall, there are still around $9$ million articles with neither a Wikipedia nor a Wikidata description.


% For the vast majority of articles that have both Wikipedia short description and Wikidata description, these two are the same up to capitalization. While it is possible to use these descriptions as a base for Wikipedia short descriptions when they exist, they can sometimes be too technical and lengthy for Wikipedia short description. In addition, most of the articles missing Wikipedia short description do not have a Wikidata description either. In~\Figref{fig:wikidata_stats} we present statistics about comparison between Wikidata and Wikipedia short descriptions. 

==> _UNUSED_04_experiments_setup.tex <==
% In this section, we briefly describe the experimental setup used to validate the model. We discuss data preprocessing, automatic evaluation, and manual evaluation.

% \subsection{Data}
% \label{ssec:data}
% \subsubsection{Data Sampling} 
% We sample Wikipedia articles from the 25 languages mBART was pre-trained on. This set covers different language families and different amount of text available for training. We collect the first paragraph of each article and its associated Wikipedia short description (if available) using Wikimedia REST API.\footnote{\url{https://en.wikipedia.org/api/rest_v1/}}
% In our experiments, for faster development cycles, we simulate a smaller Wikipedia: it consists of 100K different randomly selected Wikidata entities. 
% Each entity is associated with articles in different languages, and each article may (or not) have a short description. We selected only entities that have at least one article and one description in one of the 25 languages.
% To validate that our finding scale to the full Wikipedia scale, we re-ran the best model on full scale once and observed that the same conclusions applied.

% We also collected pre-trained knowledge graph embeddings. For each entity $E$ in our dataset, we retrieve the embedding of its parents with respect to the relation: ``instance-of''. We call it the type embedding of the entity $E$.\footnote{Knowledge graph: \url{https://dumps.wikimedia.org/wikidatawiki/entities/}}
% When an entity has multiple parents for the ``instance-of'' relation, its type embedding is obtained by averaging the embeddings of all the parents.
% When an entity does not have a parent for the ``instance-of'' relation, we use a dummy type embedding being the average over all type embeddings in our dataset.

% \subsubsection{Statistics}
% Our train set consists of 100K different Wikidata entities, while our validation set consists of 10K entities. Out of the 100K samples, 94.19\% are connected to at least one other item with the "instance-of" relation in the Wikidata graph, and as a result, has a corresponding KG type embedding. 
% In~\Figref{fig:distribution}, we show the number of entities which have articles and descriptions in other languages. Most entities only have $1$ language where they have an article and a description. Very few entities have articles and descriptions in all 25 languages.
% Overall, 61.9\% of our samples have at least one description other than the target description, these represent cases where our model can exploit extra descriptions. 76.58\% of the samples have at least one Wikipedia article other than the article we are generating the description for. As a result, in such cases, our model has a chance to exploit information from the other languages when generating the description.


% \subsection{Baselines}
% \label{ssec:baselines}
% As we introduce the task of short description generation, we built a range of baseline models to compare \name to:
% \begin{itemize}
%     \item \textbf{Simple baseline}: This model returns the first $n$ words of the article as a description. We choose $n$ as average length of description for each language.
%     \item \textbf{Translation baseline}: For the cases when we have multiple descriptions in different languages available, we translate existing description into the target language using Google Translate. If there are more than one description available, we choose the one from the largest-resource language.
%     \item \textbf{Monolingual baseline}: We train mBART using only a subset of the original training dataset that contains article and description in the desired language. We train monolingual models for all 25 languages we consider.
% \end{itemize}

% \subsection{Evaluation}
% \label{ssec:evaluation}
% \subsubsection{Automatic evaluation metrics}
% We use MoverScore~\cite{zhao-etal-2019-moverscore} for automatic evaluation because this metric better correlates with human judgments than token matching metrics like BLEU in a variety of generation tasks, including summarization. MoverScore is a metric that builds upon multilingual contextualized representations and computes the earth mover's distance in embedding space between the target and the model-generated summary. Using an automatic metric that goes beyond token matching is particularly important for abstractive summarization where many ``good'' answers with completely different word choices are possible.

% \subsubsection{Amazon Mechanical Turk}

% In addition to the automated evaluation, we perform human evaluation on Amazon Mechanical Turk. We test our model in three languages: English, Romanian, and Hindi. These languages are chosen because they belong to different language families and they have different amount of text available for training. We also had in mind the number of workers available on the platform that speak the chosen language. All three of the chosen languages are a mother tongue for a high number of workers on the platform~\cite{pavlick-etal-2014-language}. 
% We compare our model's outputs to the existing description in Wikipedia written by editors.

% \paragraph{Participants} 
% To ensure high-quality results and reasonably fast delivery of them, we approve only workers that have task approval rates greater than 99\% for English task and 97\% for Romanian and Hindi tasks. We also ask for at least 1000 previously approved tasks for the English task, and 500 for Romanian and Hindi tasks. Participants in Hindi and Romanian tasks were also restricted by location (India and Romania, respectively). We targeted a pay rate of \$8-10 per hour following the minimum wage in USA.

% \paragraph{Data sampling} To ensure workers do not have to compare the same descriptions, we remove all the samples for which our model generated the same description as the existing one, up to capitalization. This accounts for 37.5\% samples in English, 68.95\% samples in Romanian, and 64.62\% of samples in Hindi. We stratify the rest of our data by the achieved MoverScores into 10 equally-sized groups (deciles). For English task, we then randomly choose 100 samples from each decile to be presented to the workers. Because articles in Romanian and Hindi have less topic diversity than in English, to ensure that we sample uniformly over different topics in these languages, within each decile, we perform k-means++~\cite{ilprints778} style sampling. K-means++ is a seeding technique that increases the chance of choosing initial centroids that are far away from each other, and consequently, belong to different clusters. We take KG embeddings and run the k-means++ initialization. Resulting centroids are the sampled articles. This provides us with articles that are "spread out" in the embeddings space.

% \paragraph{Setting} Workers are shown the whole Wikipedia page and they are asked to choose a more appropriate description between our model's output and the ground truth. To help workers understand what an appropriate description is, we give examples of good descriptions in the instructions. These descriptions are taken manually following the guidelines for Wikipedia short descriptions\footnote{\url{https://en.wikipedia.org/wiki/Wikipedia:Short_description}}.

% \paragraph{Evaluation} One task consists of a batch of 10 samples. One of the samples is always a honeypot. This has been done to ensure that each worker runs into one honeypot while solving the task. Answers of workers that failed on more than 20\% of honeypots they ran into are filtered from the evaluation. Given the lower number of speakers of Romanian and Hindi on Amazon Mechanical Turk, to verify that our workers understand these languages, we show them a simple multiple-choice entry question that they have to solve to have their task approved. Each sample is solved by three different workers and final decision is made by majority vote. Overall, we end up with 1100 instances to be labelled for each language, each annotated 3 times for a total of 3300 annotations.


==> _UNUSED_05_experiments_results.tex <==
% \subsection{Performance evaluation}
% \label{ssec:perf_eval}

% We train and evaluate variations of \name models with and without external signals and baselines on the Wikipedia train, and validation sets described before. We train four variations: \name that only uses first paragraphs as the input (denoted as Descartes in the results), \name that in addition uses KG type embedddings (+ KG), that uses existing descriptions (+ Desc.), and the one that exploits both of the signals (+ KG \& Desc.). We report the average MoverScore on test sets in \Tabref{tab:eval-systems} for all models across the 25 languages. 

% \subsubsection{Analysis}
% \name models outperform both simple and translation baseline. While translation baseline might seem like the best way to solve this problem when other descriptions are available, the structure of these descriptions can vary in different languages. Simply translating it cannot capture such subtleties, while \name can learn these mappings and produce higher quality descriptions.

% When observing the results over different languages, it appears that low-resource languages are solved as well as high-resource ones. Scores are high for low-resource languages for a few reasons. First, this is partly due to the nature of the automatic metric we use. Embeddings from low-resource languages are placed closer in the mulitlingual embedding space, making the distances between them artificially smaller and, consequently, the differences between smaller as well. Second, Wikipedia articles in low-resource languages cover a less broad range of topics than in high-resource languages. This makes the task of generating the descriptions inherently easier for low-resource languages. Finally, we can exploit the articles in high-resource languages when generating the descriptions in low-resource efficiently.
% \name also performs similarly or better than its monolingual counterparts for all the tested languages. This means there is no performance decline in the multilingual setting and can be used as it is for both high and low-resource languages with one unified model. Some examples of generated descriptions can be seen in the~\Appref{appendix:results}.


% \subsubsection{Aggregated model comparison.}
% To compare models across all test sets, instead of blindly averaging we use the more robust paired aggregations methodology recommended by ~\newcite{peyrard-etal-2021-better}. We use their \emph{Pairformance}\footnote{\url{https://github.com/epfl-dlab/pairformance}} tool that implements a Bradley-Terry model to compute pairwise aggregated comparison of models. These results are reported in \Tabref{tab:bt-comparison}. For every pair of models (A and B), it gives the probability that model A is better than the other B based on how many instances A gets a better score than B. Because it is an instance-level pairing, this aggregation is scale-independent and more robust to outliers than averaging \cite{peyrard-etal-2021-better}. This is important in our case, because from one language to the next, MoverScore absolute values are not comparable.

% This confirms that \name model with type embeddings and existing descriptions (+KG \& Desc.) largely outperforms the simple baseline. It also performs significantly better than \name that uses only first paragraphs. It only slightly outperforms the ablated models: with just the type embedding (+KG) and with just the other description in other languages (+Desc.). It indicates that each of these two signals alone is already sufficient to solve the task fairly well. We show in the next section, that the model has little room for improvement as it is already indistinguishable from human performance. The \name model with type embeddings and existing descriptions still leverages its signals and is important for tricky corner cases. We show some examples were the KG. and/or Desc. were necessary in \Appref{appendix:results}. However, tricky corner cases are rare, and do not affect much the fully aggregated results.

% To show that \name makes meaningful use of these signals, we feed the trained models that exploit additional signals with only them, excluding the text of the article. Model that uses only existing descriptions achieves an average MoverScore of 0.651 which is similar to the performance of the translation baseline. The model that uses only KG type embeddings has a MoverScore is 0.598, which is not much higher from the simple baseline.

% \begin{table*}[t]
% \centering
% \caption{\textmd{\textbf{Automatic evaluation results.} 
% MoverScore of baselines and models reported on the validation set of each of the 25 languages considered. Note that the translation baseline was evaluated on a subset of items that have multiple descriptions available, if no other description is available the translation baseline is not applicable. This corresponds to 61.9\% of all instances.
% }}
% \resizebox{\textwidth}{!}{
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{@{}lccccccccccccccccccccccccccc@{}}
% \toprule
% & en & de & nl & es & it & ru & fr & zh & ar & vi & ja & fi & ko & tr & ro & cs & et & lt & kk & lv & hi & ne & my & si & gu & avg micro & avg macro\\
% \midrule
% \emph{\% PID with article}   & 77 & 45 & 41 & 41 & 37 & 36 & 35 & 27 & 27 & 24 & 24 & 17 & 16 & 14 & 12 & 9 & 7 & 7 & 7 & 5 & 4 & 1 & 1 & .7 & .7 & \\
% \midrule
% \midrule
% \multicolumn{3}{l}{\emph{\textbf{Baselines}}} \\ 
% \hspace{4mm} Simple  & .564 & .563 & .572 & .565 & .558 & .622 & .556 & .627 & .651 & .581 & .594 & .584 & .618 & .581 & .560 & .567 & .596 & .616 & .622 & .570 & .636 & .645 & .710 & .750 & .785 & .576 & .612\\
% \hspace{4mm} Monolingual  & .770 & \textbf{.798} & .833 & .835 & \textbf{.857} & \textbf{.827} & .810 & \textbf{.820} & .881 & .827 & \textbf{.850} & \textbf{.816} & .794 & .708 & \textbf{.907} & .793 & .887 & .889 & .591 & \textbf{.800} & .889 & .791 & .810 & \textbf{.935} & \textbf{.978} & & .827 \\
% \hspace{4mm} Translation  & .682 & .661 & .619 & .686 & .647 & .704 & .688 & .693 & .716 & .704 & .679 & .661 & .703 & .658 & .648 & .659 & .775 & .693 & .665 & .674 & .733 & .688 & .713 & .903 & .872 & .666 & .674 \\


% \midrule
% \multicolumn{3}{l}{\emph{\textbf{Proposed Models}}} \\
% \hspace{4mm} \name  & .772 & .776 & .840 & .836 & .847 & .824 & .810 & .809 & .881 & \textbf{.837} & .833 & .812 & .800 & .697 & .894 & .794 & .881 & \textbf{.892} & .614 & .753 & .888 & .771 & .772 & \textbf{.923} & .892 & .830 & .818 \\
% \hspace{4mm} + KG  & .778 & .793 & \textbf{.846} & .834 & .853 & \textbf{.824} & .816 & .812 & .879 & .825 & .841 & .814 & \textbf{.810} & .696 & .898 & .787 & .886 & .874 & .604 & \textbf{.773} & \textbf{.890} & .788 & .795 & .821 & .895 & .832 & .817\\
% \hspace{4mm} + Desc.  & .775 & .794 & .844 & \textbf{.840} & .852 & .819 & .814 & .815 & \textbf{.884} & .831 & \textbf{.842} & \textbf{.816} & .803 & \textbf{.709} & .898 & .794 & \textbf{.898} & .872 & \textbf{.653} & .756 & .891 & .780 & \textbf{.836} & .901 & .899 & .832 & .825\\
% \hspace{4mm} + KG \& Desc.  & \textbf{.781} & \textbf{.798} & \textbf{.846} & .838 & \textbf{.855} & .821 & \textbf{.825} & \textbf{.815} & .883 & .818 & .840 & .814 & .802 & .704 & \textbf{.900} & \textbf{.807} & .888 & .882 & .633 & .747 & .888 & \textbf{.800} & .835 & .862 & \textbf{.900} & .833 & .823\\

% \bottomrule                            
% \end{tabular}
% }

% \label{tab:eval-systems}
% \end{table*}




% % \begin{table*}
% % \begin{tabular}{@{}llllllll@{}}
% % \toprule
% %   & simple   & base     & type     & summary  & full     & monolingual & translate \\ \midrule
% % ar & 0.651473 & 0.880743 & 0.878912 & 0.883975 & 0.882976 &             &           \\
% % cs & 0.567099 & 0.793681 & 0.787413 & 0.794019 & 0.806547 &             &           \\
% % de & 0.563285 & 0.775796 & 0.793445 & 0.793705 & 0.797901 & 0.797678    &           \\
% % en & 0.563913 & 0.772156 & 0.778208 & 0.774876 & 0.781041 & 0.770118    &           \\
% % es & 0.564699 & 0.836054 & 0.833729 & 0.839981 & 0.837589 &             &           \\
% % et & 0.596071 & 0.880847 & 0.886005 & 0.898155 & 0.888292 &             &           \\
% % fi & 0.583562 & 0.81247  & 0.81411  & 0.81585  & 0.813693 &             &           \\
% % fr & 0.555732 & 0.810067 & 0.816261 & 0.813607 & 0.824505 & 0.809916    &           \\
% % gu & 0.78502  & 0.891714 & 0.895406 & 0.898724 & 0.899846 &             &           \\
% % hi & 0.635687 & 0.887667 & 0.890242 & 0.890994 & 0.88759  & 0.889436    &           \\
% % it & 0.558138 & 0.846738 & 0.852643 & 0.851509 & 0.854508 & 0.857418    &           \\
% % ja & 0.594074 & 0.83274  & 0.841408 & 0.841681 & 0.839891 &             &           \\
% % kk & 0.622512 & 0.61378  & 0.603529 & 0.652872 & 0.632531 &             &           \\
% % ko & 0.617996 & 0.79931  & 0.810318 & 0.8027   & 0.801885 &             &           \\
% % lt & 0.616399 & 0.892462 & 0.874005 & 0.871917 & 0.882066 &             &           \\
% % lv & 0.570078 & 0.752752 & 0.7725   & 0.756163 & 0.746779 &             &           \\
% % my & 0.709772 & 0.771921 & 0.794527 & 0.836144 & 0.83499  &             &           \\
% % ne & 0.645083 & 0.771464 & 0.788223 & 0.780299 & 0.799509 &             &           \\
% % nl & 0.572293 & 0.839823 & 0.845701 & 0.844146 & 0.845882 &             &           \\
% % ro & 0.560011 & 0.893528 & 0.897857 & 0.897854 & 0.900237 & 0.907122    &           \\
% % ru & 0.621811 & 0.823717 & 0.823838 & 0.81942  & 0.820914 &             &           \\
% % si & 0.749846 & 0.92278  & 0.821273 & 0.901357 & 0.861962 &             &           \\
% % tr & 0.580976 & 0.69681  & 0.695895 & 0.708753 & 0.703612 &             &           \\
% % vi & 0.580555 & 0.837303 & 0.825465 & 0.83076  & 0.817969 &             &           \\
% % zh & 0.626522 & 0.808892 & 0.812072 & 0.814553 & 0.814806 & 0.820444    &          \\ \bottomrule
% % \end{tabular}
% % \caption{Mover score per language}
% % \label{tab:per_lang_scores}
% % \end{table*}

% \begin{table}
% \caption{\textmd{\textbf{Paired aggregated results.} Probability that one model is better than any other across all instances, based on the Bradley-Terry aggregation model. All of the values are statistically significant ($^*$ means the probability is statistically significantly different from $0.5$ under the sign test at the $0.05$ threshold).}}
% \resizebox{\columnwidth}{!}{
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{@{}|l|c|c|c|c|c|@{}}
% \hline
%         & Simple & \name  & + KG  & + Desc. & + KG \& Desc.  \\ 
% \hline
% Simple  & -      & .077$^*$ & .076$^*$ & .076$^*$   & .075$^*$ \\
% \hline
% \name    & .923$^*$  & -     & .485$^*$ & .479$^*$   & .478$^*$ \\
% \hline
% + KG    & .924$^*$  & .515$^*$ & -     & .493   & .492 \\
% \hline
% + Desc. & .924$^*$  & .521$^*$ & .507 & -       & .499 \\
% \hline
% + KG \& Desc.    & \textbf{.925}$^*$  & \textbf{.522}$^*$ & \textbf{.508} & \textbf{.501}   & -    \\ 
% \hline
% \end{tabular}
% }
% \label{tab:bt-comparison}
% \end{table}


% \subsection{External validity}
% \label{ssec:external-val}
% \name (and its variants) intended usage is to automatically propose short descriptions for articles that do not have one. For evaluation, however, we had to create test sets based on articles that already have a short description in the real Wikipedia. Articles that already have a short description in Wikipedia might be different from the ones that do not. If that is the case, our test set might not be fully representative of articles for which our model will be deployed. In data science, this is often known as the \emph{external validity} problem.

% A common way to estimate the external validity of a model is to compute \emph{propensity scores}. The propensity score of a data point is the estimated likelihood that this data point happens to be in our test dataset.
% In our case, this means training a model to estimate the likelihood that any given article already has a description. For that, we craft a Wikipedia dataset containing articles (in English only) with and without descriptions. Then, we finetune a BERT-based classifier that maps an input article to the binary label: has a description or not. This model can predict which articles have short descriptions with an accuracy of 0.77 on a held-out test set. Then, for a given article, the classification softmax is used as the propensity score, the likelihood of having a description. Finally, we look into our test set, where all articles have descriptions but where we can evaluate the model and stratify results according to propensity scores. The average performance across different propensity scores is reported in~\Figref{fig:propensity}. Intuitively, articles with low propensity scores resemble articles that do not have descriptions, while articles with high propensity are more stereotypical of the dataset.

% As expected, \name (+KG \& Desc.) performs better for articles with high propensity (representative of the dataset). However, we see that the model performs already fairly well for the low propensity articles, with no decrease in performance compared to medium propensity. These results indicate that \name (+KG \& Desc.) is expected to perform well for articles that do not have short descriptions in Wikipedia yet.



% \begin{figure}
%   \centering
%   \includegraphics[width=0.9\columnwidth]{images/propensity_eval.pdf}
%   \caption{\textmd{\textbf{External validity.} MoverScore of \name (+KG \& Desc.) stratified across propensity scores for the English test set. Propensity score is an estimate of the probability, for an article, to have a short description. The dashed line depicts the average MoverScore of the model on the full test set (as in Table 1. first column last row)}}
%   \label{fig:propensity}
% \end{figure}



% \subsection{Human evaluation}
% \label{ssec:human-eval}

% Automatic evaluation metrics remain limited in their ability to capture output quality. Furthermore, automatic scores are only useful to compare relative improvements between models, they do not measure if the outputs are ``good enough'' to solve the task.
% Thus we also conducted a manual evaluation on Amazon Mechanical Turk for three languages: English (en), Hindi (hi), and Romanian (ro) (see \Secref{ssec:evaluation} for detailed setup).
% Human annotators were shown a Wikipedia page together with an existing human-written short description and the output of \name (+KG \& Desc.) with type embeddings and existing descriptions (in randomized order). Then they were asked which short description better fit the page. The results were stratified by MoverScore scores, so that we sample cases where our model scores \emph{high} and also where our model scores \emph{low}. These results are reported in \Figref{fig:human_eval}.

% We observe that, for most MoverScore deciles in the three languages, \name (+KG \& Desc.) is not statistically distinguishable from the human-written short descriptions. There is about a 50\% chance that our model's output is preferred. Remarkably, this holds across all automatic scores deciles. There is no correlation between automatic scores and whether humans will prefer our generated outputs or not. In part, this comes from the nature of automatic evaluation, which compares the model's output to the target human-written one. This assumes that the human-written is always correct and the only possible answer. Yet, some human-written outputs can be too short, too vague, and alternative formulations are also valid. 
% For example, in the lower scoring decile for English articles, \emph{Ain O Salish Kendro} a non-governmental human-rights organization from Bangladesh has the following descriptions: \emph{Organization} by the editor from Wikipedia and \emph{Human rights organization in Bangladesh} by \name.
% Similarly, an Indonesian island is currently described in Wikipedia by \emph{Island} whereas \name generated: \emph{island in East Nusa Tenggara, Indonesia}. These are examples where the model's output has a low score because it is different from the target despite its output being more precise (and still factually correct).

% Furthermore, these results demonstrate that \name (+KG \& Desc.) performs similarly well for all three languages despite them having very different amounts of training data.

% Finally, there are a few exceptions where ground truth is a clear winner, in particular some of the higher deciles for Romanian and English descriptions. This drop in performance is a consequence of a high number of longer descriptions in these deciles. During testing, we limited the length of the output descriptions to force our model to be concise. As a result, for particular types of articles, e.g., disambiguation pages, our model produces a description that is similar to the ground truth, but it ends abruptly. This is demonstrated by comparing \Figref{fig:human_eval}~(a) and ~(b). When we remove disambiguation pages and cases where the model was cut-off, \name (+KG \& Desc.) again bridges the gap with human-written annotations. Therefore, when used in practice, we will increase the maximum length authorized to the model and ignore disambiguation pages.



%\maxime{Figure 4,5, and 6 could be a single bar figure with a grouped bar plot, for each decile there are 3 bar one for each language (different colors)}


% \subsection{Error analysis}
% \label{ssec:err-analysis}
% To further investigate the quality of model-generated descriptions, as well as human-written ones, we manually inspect the descriptions that were not selected by Amazon Mechanical Turk workers. In other words, we inspect the descriptions generated by \name (+KG \& Desc.) when human-written ones were chosen as better for the given Wikipedia page and vice versa.

% We first adopted an iterative coding strategy, manually and independently inspecting the data to build an understanding of types of the errors that occur in the descriptions.
% We perform it as follows: each iteration, two of us independently label same 100 randomly chosen samples, 50 from the scenario where our model was preferred and 50 where human-written description was preferred. Set of labels (error categories) can be expanded in each iteration. At the end of each round, we discuss disagreements and appropriateness of the selected categories, and modify them if needed. As a stopping criterion, we decide to use average pairwise Fleiss Kappa agreement greater than 0.6. We repeated the labelling process twice, achieving the agreements of 0.55 and 0.77, respectively. The final error categories are shown in~\Tabref{tab:err-cat}. Alternatively, when no particular error was found, the description was annotated with \emph{good} category. Indeed, it happens quite often that a description, despite not being preferred by humans over another one, is still good and valid.

% Then, using this categorization, we annotate randomly chosen 300 instances, consisting of both samples where \name (+KG \& Desc.) was not the preferred one and where the human-written description was not the preferred one. We annotated the non-preferred descriptions in both cases, without knowing whether they came from our model or humans. We achieved the agreement of 0.767 and we manually resolved the disagreements. In~\Figref{fig:error-analysis}, we summarize our annotations.

% Interestingly, the profile of the mistakes made by \name (+KG \& Desc.) is similar to the ones Wikipedia editors make. Our model makes more factual errors than Wikipedia editors but never generates a too-long description due to the limited output length. In manual inspection, we realize that factual errors come from two things: (i) generating the wrong year and (ii) not using "former" for the things that are no longer true or no longer exist. The second type of error is also common for the human-written descriptions, as editors do not necessarily come back to edit the descriptions when something changes in the world. Overall, around 91.3\% of our model's descriptions were at least good enough on their own. The same applies to the editor-written descriptions (92.1\%). We believe that this analysis convincingly demonstrates that \name (+KG \& Desc.) is capable of effectively making valid descriptions with a quality similar to that of human editors.

% \begin{figure}
%   \centering
%   \includegraphics[width=0.9\columnwidth]{images/error_profiles.pdf}
%   \caption{\textmd{\textbf{Error analysis.} In (a) we report the manual error analysis performed on descriptions that were not chosen by humans in the MT annotations using the categories resulting from the iterative coding strategy. In (b), we take into account all instances including the cases where \name produced the same descriptions as humans and the cases when descriptions were preferred. In (b), we aggregated ``Too vague'', ``Formatting error'', ``Mis-focused'', and ``Too long'' into one category: ``Other errors''.  In $91.3\%$ of instances, \name either outputted the same description as human, its description was preferred over the human or it was deemed good enough. 
%   The same aggregation for human-written descriptions gives $92.1\%$.}}
%   \label{fig:error-analysis}
% \end{figure}


% \begin{table}[]
% \caption{Final error categories. \textmd{Table shows all the error categories with a brief description of each one of them.}}
% \centering
% \resizebox{\columnwidth}{!}{
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{c|p{70mm}}
% \hline
% \textbf{Error category}   & \textbf{Description}     \\ \hline \hline
% Too vague        & The description does not contain enough information to identify the entity                                                                                         \\ \hline
% Factual error    & The description contains wrong facts, for example a wrong year, nationality of a person                                                                            \\ \hline
% Formatting error & The description is not an appropriate short-description independent of its content: it contains grammatical errors, formatting problems like using ..., errors with white spaces \\ \hline
% Mis-focused      & The description is describing other entities                                                                                                                       \\ \hline
% Too long         & The description contains too many details, is too long, or made of several sentences                                                                               \\ \hline
% \end{tabular}
% }
% \label{tab:err-cat}
% \end{table}

